GraspMamba: A Mamba-based Language-driven Grasp Detection Framework with Hierarchical Feature Learning

Grasp detection is a fundamental robotic task critical to the success of many industrial applications. However, current language-driven models for this task often struggle with cluttered images, lengthy textual descriptions, or slow inference speed. We introduce GraspMamba, a new language-driven grasp detection method that employs hierarchical feature fusion with Mamba vision to tackle these challenges. By leveraging rich visual features of the Mamba-based backbone alongside textual information, our approach effectively enhances the fusion of multimodal features. GraspMamba represents the first Mamba-based grasp detection model to extract vision and language features at multiple scales, delivering robust performance and rapid inference time. Intensive experiments show that GraspMamba outperforms recent methods by a clear margin. We validate our approach through real-world robotic experiments, highlighting its fast inference speed.

==> class/reference_old.tex <==
@inproceedings{karpathy2015deep,
  title={Deep visual-semantic alignments for generating image descriptions},
  author={Karpathy, Andrej and Fei-Fei, Li},
  booktitle={CVPR},
  year={2015}
}
@article{faghri2017vse++,
  title={Vse++: Improving visual-semantic embeddings with hard negatives},
  author={Faghri, Fartash and Fleet, David J and Kiros, Jamie Ryan and Fidler, Sanja},
  journal={arXiv preprint arXiv:1707.05612},
  year={2017}
}
@article{wang2019learning,
  title={Learning two-branch neural networks for image-text matching tasks},
  author={Wang, Liwei and Li, Yin and Huang, Jing and Lazebnik, Svetlana},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2018},
}
@inproceedings{li2019visual,
  title={Visual semantic reasoning for image-text matching},
  author={Li, Kunpeng and Zhang, Yulun and Li, Kai and Li, Yuanyuan and Fu, Yun},
  booktitle={ICCV},
  year={2019}
}
@inproceedings{yang2021sat,
  title={Sat: 2d semantics assisted training for 3d visual grounding},
  author={Yang, Zhengyuan and Zhang, Songyang and Wang, Liwei and Luo, Jiebo},
  booktitle={ICCV},
  year={2021}
}
@inproceedings{radford2021learning,
  title={Learning transferable visual models from natural language supervision},
  author={Radford, Alec and Kim, Jong Wook and Hallacy, Chris and Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and Sastry, Girish and Askell, Amanda and Mishkin, Pamela and Clark, Jack and others},
  booktitle={ICML},
  year={2021},
}
@article{chu2018real,
  title={Real-world multiobject, multigrasp detection},
  author={Chu, Fu-Jen and Xu, Ruinian and Vela, Patricio A},
  journal={IEEE Robotics and Automation Letters},
  year={2018},
}
@inproceedings{roiGrasp2019,
  title={ROI-based Robotic Grasp Detection for Object Overlapping Scenes},
  author={Zhang, Hanbo and Lan, Xuguang and Bai, Site and Zhou, Xinwen and Tian, Zhiqiang and Zheng, Nanning},
  booktitle={IROS},
  year={2019},
}
@article{dosovitskiy2020image,
  title={An image is worth 16x16 words: Transformers for image recognition at scale},
  author={Dosovitskiy, Alexey and Beyer, Lucas and Kolesnikov, Alexander and Weissenborn, Dirk and Zhai, Xiaohua and Unterthiner, Thomas and Dehghani, Mostafa and Minderer, Matthias and Heigold, Georg and Gelly, Sylvain and others},
  journal={arXiv preprint arXiv:2010.11929},
  year={2020}
}
@article{devlin2018bert,
  title={Bert: Pre-training of deep bidirectional transformers for language understanding},
  author={Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  journal={arXiv preprint arXiv:1810.04805},
  year={2018}
}
@article{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  journal={NeurIPS},
  year={2017}
}
@article{hendrycks2016gaussian,
  title={Gaussian error linear units (gelus)},
  author={Hendrycks, Dan and Gimpel, Kevin},
  journal={arXiv preprint arXiv:1606.08415},
  year={2016}
}
@article{ba2016layer,
  title={Layer normalization},
  author={Ba, Jimmy Lei and Kiros, Jamie Ryan and Hinton, Geoffrey E},
  journal={arXiv preprint arXiv:1607.06450},
  year={2016}
}
@article{alayrac2020self,
  title={Self-supervised multimodal versatile networks},
  author={Alayrac, Jean-Baptiste and Recasens, Adria and Schneider, Rosalia and Arandjelovi{\'c}, Relja and Ramapuram, Jason and De Fauw, Jeffrey and Smaira, Lucas and Dieleman, Sander and Zisserman, Andrew},
  journal={NeurIPS},
  year={2020}
}
@inproceedings{xiang2021learning,
  title={Learning rgb-d feature embeddings for unseen object instance segmentation},
  author={Xiang, Yu and Xie, Christopher and Mousavian, Arsalan and Fox, Dieter},
  booktitle={CoRL},
  year={2021},
}
@inproceedings{back2022unseen,
  title={Unseen object amodal instance segmentation via hierarchical occlusion modeling},
  author={Back, Seunghyeok and Lee, Joosoon and Kim, Taewon and Noh, Sangjun and Kang, Raeyoung and Bak, Seongho and Lee, Kyoobin},
  booktitle={ICRA},
  year={2022},
}
@inproceedings{ainetter2021end,
  title={End-to-end trainable deep neural network for robotic grasp detection and semantic segmentation from rgb},
  author={Ainetter, Stefan and Fraundorfer, Friedrich},
  booktitle={ICRA},
  year={2021},
}
@inproceedings{depierre2018jacquard,
  title={Jacquard: A large scale dataset for robotic grasp detection},
  author={Depierre, Amaury and Dellandr{\'e}a, Emmanuel and Chen, Liming},
  booktitle={IROS},
  year={2018},
}
@inproceedings{fang1billion,
  title={1Billion: A Large-Scale Benchmark for General Object Grasping. in 2020 IEEE},
  author={Fang, HS and Wang, C and Gou, M and Lu, C GraspNet},
  booktitle={CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  year= {2020}
}
@article{xu2023joint,
  title={A Joint Modeling of Vision-Language-Action for Target-oriented Grasping in Clutter},
  author={Xu, Kechun and Zhao, Shuqi and Zhou, Zhongxiang and Li, Zizhang and Pi, Huaijin and Zhu, Yifeng and Wang, Yue and Xiong, Rong},
  journal={arXiv preprint arXiv:2302.12610},
  year={2023}
}
@article{yang2023pave,
  title={Pave the Way to Grasp Anything: Transferring Foundation Models for Universal Pick-Place Robots},
  author={Yang, Jiange and Tan, Wenhui and Jin, Chuhao and Liu, Bei and Fu, Jianlong and Song, Ruihua and Wang, Limin},
  journal={arXiv preprint arXiv:2306.05716},
  year={2023}
}
@inproceedings{brohan2023can,
  title={Do as i can, not as i say: Grounding language in robotic affordances},
  author={Brohan, Anthony and Chebotar, Yevgen and Finn, Chelsea and Hausman, Karol and Herzog, Alexander and Ho, Daniel and Ibarz, Julian and Irpan, Alex and Jang, Eric and Julian, Ryan and others},
  booktitle={Conference on Robot Learning},
  year={2023},
}
@inproceedings{liu2023target,
  title={Target-Referenced Reactive Grasping for Dynamic Objects},
  author={Liu, Jirong and Zhang, Ruo and Fang, Hao-Shu and Gou, Minghao and Fang, Hongjie and Wang, Chenxi and Xu, Sheng and Yan, Hengxu and Lu, Cewu},
  booktitle={CVPR},
  year={2023}
}
@article{liu2023grounding,
  title={Grounding dino: Marrying dino with grounded pre-training for open-set object detection},
  author={Liu, Shilong and Zeng, Zhaoyang and Ren, Tianhe and Li, Feng and Zhang, Hao and Yang, Jie and Li, Chunyuan and Yang, Jianwei and Su, Hang and Zhu, Jun and others},
  journal={arXiv preprint arXiv:2303.05499},
  year={2023}
}

@inproceedings{xu2023object,
  title={Object-centric Inference for Language Conditioned Placement: A Foundation Model based Approach},
  author={Xu, Zhixuan and Xu, Kechun and Xiong, Rong and Wang, Yue},
  booktitle={ICARM},
  year={2023}
}
@article{lee2022task,
  title={Task allocation and planning for product disassembly with human--robot collaboration},
  author={Lee, Meng-Lun and Behdad, Sara and Liang, Xiao and Zheng, Minghui},
  journal={Robotics and Computer-Integrated Manufacturing},
  year={2022}
}
@article{zheng2022vlmbench,
  title={Vlmbench: A compositional benchmark for vision-and-language manipulation},
  author={Zheng, Kaizhi and Chen, Xiaotong and Jenkins, Odest Chadwicke and Wang, Xin},
  journal={NeurIPS},
  year={2022}
}
@inproceedings{pinto2016supersizing,
  title={Supersizing self-supervision: Learning to grasp from 50k tries and 700 robot hours},
  author={Pinto, Lerrel and Gupta, Abhinav},
  booktitle={2016 IEEE international conference on robotics and automation (ICRA)},
  pages={3406--3413},
  year={2016},
  organization={IEEE}
}

@inproceedings{mahler2017learning,
  title={Learning deep policies for robot bin picking by simulating robust grasping sequences},
  author={Mahler, Jeffrey and Goldberg, Ken},
  booktitle={Conference on robot learning},
  pages={515--524},
  year={2017},
  organization={PMLR}
}

@article{mahler2017dex,
  title={Dex-net 2.0: Deep learning to plan robust grasps with synthetic point clouds and analytic grasp metrics},
  author={Mahler, Jeffrey and Liang, Jacky and Niyaz, Sherdil and Laskey, Michael and Doan, Richard and Liu, Xinyu and Ojea, Juan Aparicio and Goldberg, Ken},
  journal={arXiv preprint arXiv:1703.09312},
  year={2017}
}

@inproceedings{kalashnikov2018scalable,
  title={Scalable deep reinforcement learning for vision-based robotic manipulation},
  author={Kalashnikov, Dmitry and Irpan, Alex and Pastor, Peter and Ibarz, Julian and Herzog, Alexander and Jang, Eric and Quillen, Deirdre and Holly, Ethan and Kalakrishnan, Mrinal and Vanhoucke, Vincent and others},
  booktitle={Conference on Robot Learning},
  pages={651--673},
  year={2018},
  organization={PMLR}
}

@incollection{ten2018using,
  title={Using geometry to detect grasp poses in 3d point clouds},
  author={Ten Pas, Andreas and Platt, Robert},
  booktitle={Robotics research},
  pages={307--324},
  year={2018},
  publisher={Springer}
}

@inproceedings{fang2020graspnet,
  title={Graspnet-1billion: A large-scale benchmark for general object grasping},
  author={Fang, Hao-Shu and Wang, Chenxi and Gou, Minghao and Lu, Cewu},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={11444--11453},
  year={2020}
}

@inproceedings{sundermeyer2021contact,
  title={Contact-graspnet: Efficient 6-dof grasp generation in cluttered scenes},
  author={Sundermeyer, Martin and Mousavian, Arsalan and Triebel, Rudolph and Fox, Dieter},
  booktitle={2021 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={13438--13444},
  year={2021},
  organization={IEEE}
}

@inproceedings{wang2021graspness,
  title={Graspness discovery in clutters for fast and accurate grasp detection},
  author={Wang, Chenxi and Fang, Hao-Shu and Gou, Minghao and Fang, Hongjie and Gao, Jin and Lu, Cewu},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={15964--15973},
  year={2021}
}

@article{son2022grasping,
  title={Grasping as Inference: Reactive Grasping in Heavily Cluttered Environment},
  author={Son, Dongwon},
  journal={arXiv preprint arXiv:2205.13146},
  year={2022}
}

@inproceedings{laskey2016robot,
  title={Robot grasping in clutter: Using a hierarchy of supervisors for learning from demonstrations},
  author={Laskey, Michael and Lee, Jonathan and Chuck, Caleb and Gealy, David and Hsieh, Wesley and Pokorny, Florian T and Dragan, Anca D and Goldberg, Ken},
  booktitle={2016 IEEE international conference on automation science and engineering (CASE)},
  pages={827--834},
  year={2016},
  organization={IEEE}
}

@article{sun2021gater,
  title={GATER: Learning Grasp-Action-Target Embeddings and Relations for Task-Specific Grasping},
  author={Sun, Ming and Gao, Yue},
  journal={IEEE Robotics and Automation Letters},
  volume={7},
  number={1},
  pages={618--625},
  year={2021},
  publisher={IEEE}
}

@inproceedings{murali20206,
  title={6-dof grasping for target-driven object manipulation in clutter},
  author={Murali, Adithyavairavan and Mousavian, Arsalan and Eppner, Clemens and Paxton, Chris and Fox, Dieter},
  booktitle={2020 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={6232--6238},
  year={2020},
  organization={IEEE}
}

@inproceedings{fang2018multi,
  title={Multi-task domain adaptation for deep learning of instance grasping from simulation},
  author={Fang, Kuan and Bai, Yunfei and Hinterstoisser, Stefan and Savarese, Silvio and Kalakrishnan, Mrinal},
  booktitle={2018 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={3516--3523},
  year={2018},
  organization={IEEE}
}

@inproceedings{jang2017end,
  title={End-to-End Learning of Semantic Grasping},
  author={Jang, Eric and Vijayanarasimhan, Sudheendra and Pastor, Peter and Ibarz, Julian and Levine, Sergey},
  booktitle={Conference on Robot Learning},
  pages={119--132},
  year={2017},
  organization={PMLR}
}

@article{zeng2022robotic,
  title={Robotic pick-and-place of novel objects in clutter with multi-affordance grasping and cross-domain image matching},
  author={Zeng, Andy and Song, Shuran and Yu, Kuan-Ting and Donlon, Elliott and Hogan, Francois R and Bauza, Maria and Ma, Daolin and Taylor, Orion and Liu, Melody and Romo, Eudald and others},
  journal={The International Journal of Robotics Research},
  volume={41},
  number={7},
  pages={690--705},
  year={2022},
  publisher={SAGE Publications Sage UK: London, England}
}

@inproceedings{kiatos2019robust,
  title={Robust object grasping in clutter via singulation},
  author={Kiatos, Marios and Malassiotis, Sotiris},
  booktitle={2019 International Conference on Robotics and Automation (ICRA)},
  pages={1596--1600},
  year={2019},
  organization={IEEE}
}

@inproceedings{kurenkov2020visuomotor,
  title={Visuomotor mechanical search: Learning to retrieve target objects in clutter},
  author={Kurenkov, Andrey and Taglic, Joseph and Kulkarni, Rohun and Dominguez-Kuhne, Marcus and Garg, Animesh and Mart{\'\i}n-Mart{\'\i}n, Roberto and Savarese, Silvio},
  booktitle={2020 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={8408--8414},
  year={2020},
  organization={IEEE}
}

@inproceedings{danielczuk2019mechanical,
  title={Mechanical search: Multi-step retrieval of a target object occluded by clutter},
  author={Danielczuk, Michael and Kurenkov, Andrey and Balakrishna, Ashwin and Matl, Matthew and Wang, David and Mart{\'\i}n-Mart{\'\i}n, Roberto and Garg, Animesh and Savarese, Silvio and Goldberg, Ken},
  booktitle={2019 International Conference on Robotics and Automation (ICRA)},
  pages={1614--1621},
  year={2019},
  organization={IEEE}
}

@article{yang2020deep,
  title={A deep learning approach to grasping the invisible},
  author={Yang, Yang and Liang, Hengyue and Choi, Changhyun},
  journal={IEEE Robotics and Automation Letters},
  volume={5},
  number={2},
  pages={2232--2239},
  year={2020},
  publisher={IEEE}
}

@article{xu2021efficient,
  title={Efficient learning of goal-oriented push-grasping synergy in clutter},
  author={Xu, Kechun and Yu, Hongxiang and Lai, Qianen and Wang, Yue and Xiong, Rong},
  journal={IEEE Robotics and Automation Letters},
  volume={6},
  number={4},
  pages={6337--6344},
  year={2021},
  publisher={IEEE}
}

@article{huang2021visual,
  title={Visual foresight trees for object retrieval from clutter with nonprehensile rearrangement},
  author={Huang, Baichuan and Han, Shuai D and Yu, Jingjin and Boularias, Abdeslam},
  journal={IEEE Robotics and Automation Letters},
  volume={7},
  number={1},
  pages={231--238},
  year={2021},
  publisher={IEEE}
}

@article{stepputtis2020language,
  title={Language-conditioned imitation learning for robot manipulation tasks},
  author={Stepputtis, Simon and Campbell, Joseph and Phielipp, Mariano and Lee, Stefan and Baral, Chitta and Ben Amor, Heni},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={13139--13150},
  year={2020}
}

@inproceedings{shridhar2022cliport,
  title={Cliport: What and where pathways for robotic manipulation},
  author={Shridhar, Mohit and Manuelli, Lucas and Fox, Dieter},
  booktitle={Conference on Robot Learning},
  pages={894--906},
  year={2022},
  organization={PMLR}
}

@inproceedings{rao2018learning,
  title={Learning robotic grasping strategy based on natural-language object descriptions},
  author={Rao, Achyutha Bharath and Krishnan, Krishna and He, Hongsheng},
  booktitle={2018 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={882--887},
  year={2018},
  organization={IEEE}
}

@inproceedings{chen2021joint,
  title={A joint network for grasp detection conditioned on natural language commands},
  author={Chen, Yiye and Xu, Ruinian and Lin, Yunzhi and Vela, Patricio A},
  booktitle={2021 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={4576--4582},
  year={2021},
  organization={IEEE}
}

@inproceedings{ito2022integrated,
  title={Integrated Learning of Robot Motion and Sentences: Real-Time Prediction of Grasping Motion and Attention based on Language Instructions},
  author={Ito, Hiroshi and Ichiwara, Hideyuki and Yamamoto, Kenjiro and Mori, Hiroki and Ogata, Tetsuya},
  booktitle={2022 International Conference on Robotics and Automation (ICRA)},
  pages={5404--5410},
  year={2022},
  organization={IEEE}
}

@article{misra2016tell,
  title={Tell me dave: Context-sensitive grounding of natural language to manipulation instructions},
  author={Misra, Dipendra K and Sung, Jaeyong and Lee, Kevin and Saxena, Ashutosh},
  journal={The International Journal of Robotics Research},
  volume={35},
  number={1-3},
  pages={281--300},
  year={2016},
  publisher={SAGE Publications Sage UK: London, England}
}

@article{brown2020language,
  title={Language models are few-shot learners},
  author={Brown, Tom and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared D and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and others},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={1877--1901},
  year={2020}
}


@inproceedings{stengel2022guiding,
  title={Guiding Multi-Step Rearrangement Tasks with Natural Language Instructions},
  author={Stengel-Eskin, Elias and Hundt, Andrew and He, Zhuohong and Murali, Aditya and Gopalan, Nakul and Gombolay, Matthew and Hager, Gregory},
  booktitle={Conference on Robot Learning},
  pages={1486--1501},
  year={2022},
  organization={PMLR}
}

@article{ahn2022can,
  title={Do as i can, not as i say: Grounding language in robotic affordances},
  author={Ahn, Michael and Brohan, Anthony and Brown, Noah and Chebotar, Yevgen and Cortes, Omar and David, Byron and Finn, Chelsea and Gopalakrishnan, Keerthana and Hausman, Karol and Herzog, Alex and others},
  journal={arXiv preprint arXiv:2204.01691},
  year={2022}
}

@article{huang2022inner,
  title={Inner Monologue: Embodied Reasoning through Planning with Language Models},
  author={Huang, Wenlong and Xia, Fei and Xiao, Ted and Chan, Harris and Liang, Jacky and Florence, Pete and Zeng, Andy and Tompson, Jonathan and Mordatch, Igor and Chebotar, Yevgen and others},
  journal={arXiv preprint arXiv:2207.05608},
  year={2022}
}

@article{shridhar2018interactive,
  title={Interactive visual grounding of referring expressions for human-robot interaction},
  author={Shridhar, Mohit and Hsu, David},
  journal={arXiv preprint arXiv:1806.03831},
  year={2018}
}


@article{ahn2018interactive,
  title={Interactive text2pickup networks for natural language-based human--robot collaboration},
  author={Ahn, Hyemin and Choi, Sungjoon and Kim, Nuri and Cha, Geonho and Oh, Songhwai},
  journal={IEEE Robotics and Automation Letters},
  volume={3},
  number={4},
  pages={3308--3315},
  year={2018},
  publisher={IEEE}
}

@inproceedings{hatori2018interactively,
  title={Interactively picking real-world objects with unconstrained spoken language instructions},
  author={Hatori, Jun and Kikuchi, Yuta and Kobayashi, Sosuke and Takahashi, Kuniyuki and Tsuboi, Yuta and Unno, Yuya and Ko, Wilson and Tan, Jethro},
  booktitle={2018 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={3774--3781},
  year={2018},
  organization={IEEE}
}

@article{zhang2021invigorate,
  title={Invigorate: Interactive visual grounding and grasping in clutter},
  author={Zhang, Hanbo and Lu, Yunfan and Yu, Cunjun and Hsu, David and La, Xuguang and Zheng, Nanning},
  journal={arXiv preprint arXiv:2108.11092},
  year={2021}
}

@inproceedings{goodwin2022semantically,
  title={Semantically grounded object matching for robust robotic scene rearrangement},
  author={Goodwin, Walter and Vaze, Sagar and Havoutis, Ioannis and Posner, Ingmar},
  booktitle={2022 International Conference on Robotics and Automation (ICRA)},
  pages={11138--11144},
  year={2022},
  organization={IEEE}
}

@article{yang2022interactive,
  title={Interactive Robotic Grasping with Attribute-Guided Disambiguation},
  author={Yang, Yang and Lou, Xibai and Choi, Changhyun},
  journal={arXiv preprint arXiv:2203.08037},
  year={2022}
}

@inproceedings{yu2016modeling,
  title={Modeling context in referring expressions},
  author={Yu, Licheng and Poirson, Patrick and Yang, Shan and Berg, Alexander C and Berg, Tamara L},
  booktitle={European Conference on Computer Vision},
  pages={69--85},
  year={2016},
  organization={Springer}
}

@inproceedings{mildenhall2020nerf,
  title={NeRF: Representing Scenes as Neural Radiance Fields for View Synthesis},
  author={Mildenhall, Ben and Srinivasan, Pratul P and Tancik, Matthew and Barron, Jonathan T and Ramamoorthi, Ravi and Ng, Ren},
  booktitle={Computer Vision--ECCV 2020: 16th European Conference, Glasgow, UK, August 23--28, 2020, Proceedings, Part I},
  pages={405--421},
  year={2020}
}

@article{haarnoja2018soft,
  title={Soft actor-critic algorithms and applications},
  author={Haarnoja, Tuomas and Zhou, Aurick and Hartikainen, Kristian and Tucker, George and Ha, Sehoon and Tan, Jie and Kumar, Vikash and Zhu, Henry and Gupta, Abhishek and Abbeel, Pieter and others},
  journal={arXiv preprint arXiv:1812.05905},
  year={2018}
}

@article{christodoulou2019soft,
  title={Soft actor-critic for discrete action settings},
  author={Christodoulou, Petros},
  journal={arXiv preprint arXiv:1910.07207},
  year={2019}
}

@MISC{coumans2021,
author =   {Erwin Coumans and Yunfei Bai},
title =    {PyBullet, a Python module for physics simulation for games, robotics and machine learning},
howpublished = {\url{http://pybullet.org}},
year = {2016--2021}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@inproceedings{perez2018film,
  title={Film: Visual reasoning with a general conditioning layer},
  author={Perez, Ethan and Strub, Florian and De Vries, Harm and Dumoulin, Vincent and Courville, Aaron},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={32},
  number={1},
  year={2018}
}

@article{liu2021ocrtoc,
  title={OCRTOC: A cloud-based competition and benchmark for robotic grasping and manipulation},
  author={Liu, Ziyuan and Liu, Wei and Qin, Yuzhe and Xiang, Fanbo and Gou, Minghao and Xin, Songyan and Roa, Maximo A and Calli, Berk and Su, Hao and Sun, Yu and others},
  journal={IEEE Robotics and Automation Letters},
  volume={7},
  number={1},
  pages={486--493},
  year={2021},
  publisher={IEEE}
}


@Misc{appendix,
author = {Xu, Kechun},
title = {Paper with appendix},
howpublished={\url{https://drive.google.com/file/d/1WBYInZAioPsFZ8sJHvGirV36a1ifXz9F/view}},
year={2022},
}

@Misc{appendix_arxiv,
author = {K. Xu},
title = {Paper with appendix},
howpublished={\url{https://arxiv.org/abs/2302.12610}},
year={2021},
}

@article{morrison2018closing,
  title={Closing the loop for robotic grasping: A real-time, generative grasp synthesis approach},
  author={Morrison, Douglas and Corke, Peter and Leitner, J{\"u}rgen},
  journal={arXiv preprint arXiv:1804.05172},
  year={2018}
}
@article{sun2021research,
  title={Research challenges and progress in robotic grasping and manipulation competitions},
  author={Sun, Yu and Falco, Joe and Roa, M{\'a}ximo A and Calli, Berk},
  journal={IEEE Robotics and Automation Letters},
  year={2021},
}
@inproceedings{tang2023selective,
  title={Selective object rearrangement in clutter},
  author={Tang, Bingjie and Sukhatme, Gaurav S},
  booktitle={CoRL},
  year={2023},
}
@article{wei2023discriminative,
  title={Discriminative Active Learning for Robotic Grasping in Cluttered Scene},
  author={Wei, Boyan and Ye, Xianfeng and Long, Chengjiang and Du, Zhenjun and Li, Bangyu and Yin, Baocai and Yang, Xin},
  journal={IEEE Robotics and Automation Letters},
  year={2023},
}
@article{gilles2023metagraspnetv2,
  title={MetaGraspNetV2: All-in-one dataset enabling fast and reliable robotic bin picking via object relationship reasoning and dexterous grasping},
  author={Gilles, Maximilian and Chen, Yuhao and Zeng, Emily Zhixuan and Wu, Yifan and Furmans, Kai and Wong, Alexander and Rayyes, Rania},
  journal={IEEE Transactions on Automation Science and Engineering},
  year={2023},
}
@inproceedings{shah2023lm,
  title={Lm-nav: Robotic navigation with large pre-trained models of language, vision, and action},
  author={Shah, Dhruv and Osi{\'n}ski, B{\l}a{\.z}ej and Levine, Sergey and others},
  booktitle={CoRL},
  year={2023},}

@article{vuong2023grasp,
  title={Grasp-anything: Large-scale grasp dataset from foundation models},
  author={Vuong, An Dinh and Vu, Minh Nhat and Le, Hieu and Huang, Baoru and Huynh, Binh and Vo, Thieu and Kugi, Andreas and Nguyen, Anh},
  journal={arXiv preprint arXiv:2309.09818},
  year={2023}
}
@article{platt2023grasp,
  title={Grasp learning: Models, methods, and performance},
  author={Platt, Robert},
  journal={Annual Review of Control, Robotics, and Autonomous Systems},
  year={2023},
}
@inproceedings{song2023llm,
  title={Llm-planner: Few-shot grounded planning for embodied agents with large language models},
  author={Song, Chan Hee and Wu, Jiaman and Washington, Clayton and Sadler, Brian M and Chao, Wei-Lun and Su, Yu},
  booktitle={ICCV},
  year={2023}
}
@article{mu2023embodiedgpt,
  title={Embodiedgpt: Vision-language pre-training via embodied chain of thought},
  author={Mu, Yao and Zhang, Qinglong and Hu, Mengkang and Wang, Wenhai and Ding, Mingyu and Jin, Jun and Wang, Bin and Dai, Jifeng and Qiao, Yu and Luo, Ping},
  journal={arXiv preprint arXiv:2305.15021},
  year={2023}
}
@article{driess2023palm,
  title={Palm-e: An embodied multimodal language model},
  author={Driess, Danny and Xia, Fei and Sajjadi, Mehdi SM and Lynch, Corey and Chowdhery, Aakanksha and Ichter, Brian and Wahid, Ayzaan and Tompson, Jonathan and Vuong, Quan and Yu, Tianhe and others},
  journal={arXiv preprint arXiv:2303.03378},
  year={2023}
}
@article{jatavallabhula2023conceptfusion,
  title={Conceptfusion: Open-set multimodal 3d mapping},
  author={Jatavallabhula, Krishna Murthy and Kuwajerwala, Alihusein and Gu, Qiao and Omama, Mohd and Chen, Tao and Maalouf, Alaa and Li, Shuang and Iyer, Ganesh and Saryazdi, Soroush and Keetha, Nikhil and others},
  journal={arXiv preprint arXiv:2302.07241},
  year={2023}
}
@inproceedings{mu2023ec2,
  title={EC2: Emergent Communication for Embodied Control},
  author={Mu, Yao and Yao, Shunyu and Ding, Mingyu and Luo, Ping and Gan, Chuang},
  booktitle={CVPR},
  year={2023}
}
@inproceedings{kumra2020antipodal,
  title={Antipodal robotic grasping using generative residual convolutional neural network},
  author={Kumra, Sulabh and Joshi, Shirin and Sahin, Ferat},
  booktitle={IROS},
  year={2020},
}
@article{beck2023singularity,
  title={Singularity avoidance with application to online trajectory optimization for serial manipulators},
  author={Beck, Florian and Vu, Minh Nhat and Hartl-Nesic, Christian and Kugi, Andreas},
  journal={IFAC-PapersOnLine},
  year={2023},
}
@article{vu2023machine,
  title={Machine learning-based framework for optimally solving the analytical inverse kinematics for redundant manipulators},
  author={Vu, Minh Nhat and Beck, Florian and Schwegel, Michael and Hartl-Nesic, Christian and Nguyen, Anh and Kugi, Andreas},
  journal={Mechatronics},
  year={2023},
}

@misc{chatgpt,
  author = {OpenAI},
  title = {{Introducing ChatGPT}},
  howpublished = {Software},
  note = {Accessed: February 6th 2023.},
}
@inproceedings{zhou2022conditional,
  title={Conditional prompt learning for vision-language models},
  author={Zhou, Kaiyang and Yang, Jingkang and Loy, Chen Change and Liu, Ziwei},
  booktitle={CVPR},
  year={2022}
}
@article{van2008visualizing,
  title={Visualizing data using t-SNE.},
  author={Van der Maaten, Laurens and Hinton, Geoffrey},
  journal={Journal of Machine Learning Research},
  year={2008}
}
@inproceedings{maitin2010cloth,
  title={Cloth grasp point detection based on multiple-view geometric cues with application to robotic towel folding},
  author={Maitin-Shepard, Jeremy and Cusumano-Towner, Marco and Lei, Jinna and Abbeel, Pieter},
  booktitle={ICRA},
  year={2010},
}
@inproceedings{domae2014fast,
  title={Fast graspability evaluation on single depth maps for bin picking with general grippers},
  author={Domae, Yukiyasu and Okuda, Haruhisa and Taguchi, Yuichi and Sumi, Kazuhiko and Hirai, Takashi},
  booktitle={ICRA},
  year={2014}
}
@article{roa2015grasp,
  title={Grasp quality measures: review and performance},
  author={Roa, M{\'a}ximo A and Su{\'a}rez, Ra{\'u}l},
  journal={Autonomous Robots},
  year={2015}
}
@article{morrison2020learning,
  title={Learning robust, real-time, reactive robotic grasping},
  author={Morrison, Douglas and Corke, Peter and Leitner, J{\"u}rgen},
  journal={The International Journal of Robotics Research},
  year={2020},
}
@inproceedings{jiang2011efficient,
  title={Efficient grasping from rgbd images: Learning using a new rectangle representation},
  author={Jiang, Yun and Moseson, Stephen and Saxena, Ashutosh},
  booktitle={ICRA},
  year={2011}
}
@article{lenz2015deep,
  title={Deep learning for detecting robotic grasps},
  author={Lenz, Ian and Lee, Honglak and Saxena, Ashutosh},
  journal={The International Journal of Robotics Research},
  year={2015},
}
@inproceedings{jiang2011efficient_cornell,
  title={Efficient grasping from rgbd images: Learning using a new rectangle representation},
  author={Jiang, Yun and Moseson, Stephen and Saxena, Ashutosh},
  booktitle={ICRA},
  year={2011}
}
@inproceedings{lu2023vl,
  title={VL-Grasp: a 6-Dof Interactive Grasp Policy for Language-Oriented Objects in Cluttered Indoor Scenes},
  author={Lu, Yuhao and Fan, Yixuan and Deng, Beixing and Liu, Fangfu and Li, Yali and Wang, Shengjin},
  booktitle={IROS},
  year={2023}
}
@inproceedings{sun2023language,
  title={Language Guided Robotic Grasping with Fine-Grained Instructions},
  author={Sun, Qiang and Lin, Haitao and Fu, Ying and Fu, Yanwei and Xue, Xiangyang},
  booktitle={IROS},
  year={2023}
}
@article{tang2023task,
  title={Task-Oriented Grasp Prediction with Visual-Language Inputs},
  author={Tang, Chao and Huang, Dehao and Meng, Lingxiao and Liu, Weiyu and Zhang, Hong},
  journal={arXiv preprint arXiv:2302.14355},
  year={2023}
}
@inproceedings{cheang2022learning,
  title={Learning 6-DoF Object Poses to Grasp Category-Level Objects by Language Instructions},
  author={Cheang, Chilam and Lin, Haitao and Fu, Yanwei and Xue, Xiangyang},
  booktitle={ICRA},
  year={2022}
}
@inproceedings{yang2021attribute,
  title={Attribute-based robotic grasping with one-grasp adaptation},
  author={Yang, Yang and Liu, Yuanhao and Liang, Hengyue and Lou, Xibai and Choi, Changhyun},
  booktitle={ICRA},
  year={2021},
}
@article{song2022human,
  title={Human-in-the-loop Robotic Grasping using BERT Scene Representation},
  author={Song, Yaoxian and Sun, Penglei and Fang, Pengfei and Yang, Linyi and Xiao, Yanghua and Zhang, Yue},
  journal={arXiv preprint arXiv:2209.14026},
  year={2022}
}
@article{tziafas2023language,
  title={Language-guided Robot Grasping: CLIP-based Referring Grasp Synthesis in Clutter},
  author={Tziafas, Georgios and Xu, Yucheng and Goel, Arushi and Kasaei, Mohammadreza and Li, Zhibin and Kasaei, Hamidreza},
  journal={arXiv preprint arXiv:2311.05779},
  year={2023}
}
@article{wang2022transformer,
  title={When transformer meets robotic grasping: Exploits context for efficient grasp detection},
  author={Wang, Shaochen and Zhou, Zhangli and Kan, Zhen},
  journal={IEEE Robotics and Automation Letters},
  year={2022},
}
@inproceedings{yang2020learning,
  title={Learning texture transformer network for image super-resolution},
  author={Yang, Fuzhi and Yang, Huan and Fu, Jianlong and Lu, Hongtao and Guo, Baining},
  booktitle={CVPR},
  year={2020}
}
@inproceedings{carion2020end,
  title={End-to-end object detection with transformers},
  author={Carion, Nicolas and Massa, Francisco and Synnaeve, Gabriel and Usunier, Nicolas and Kirillov, Alexander and Zagoruyko, Sergey},
  booktitle={ECCV},
  year={2020}
}
@article{sun2019learning,
  title={Learning video representations using contrastive bidirectional transformer},
  author={Sun, Chen and Baradel, Fabien and Murphy, Kevin and Schmid, Cordelia},
  journal={arXiv preprint arXiv:1906.05743},
  year={2019}
}
@inproceedings{chen2020uniter,
  title={Uniter: Universal image-text representation learning},
  author={Chen, Yen-Chun and Li, Linjie and Yu, Licheng and El Kholy, Ahmed and Ahmed, Faisal and Gan, Zhe and Cheng, Yu and Liu, Jingjing},
  booktitle={ECCV},
  year={2020}
}
@article{luo2020univilm,
  title={Univilm: A unified video and language pre-training model for multimodal understanding and generation},
  author={Luo, Huaishao and Ji, Lei and Shi, Botian and Huang, Haoyang and Duan, Nan and Li, Tianrui and Chen, Xilin and Zhou, Ming},
  journal={arXiv preprint arXiv:2002.06353},
  year={2020}
}
@inproceedings{dosovitskiy2021an,
title={An Image is Worth 16x16 Words: Transformers for Image Recognition at Scale},
author={Alexey Dosovitskiy and Lucas Beyer and Alexander Kolesnikov and Dirk Weissenborn and Xiaohua Zhai and Thomas Unterthiner and Mostafa Dehghani and Matthias Minderer and Georg Heigold and Sylvain Gelly and Jakob Uszkoreit and Neil Houlsby},
booktitle={ICLR},
year={2021}
}
@article{touvron2020training,
  title={Training data-efficient image transformers \& distillation through attention},
  author={Touvron, Hugo and Cord, Matthieu and Douze, Matthijs and Massa, Francisco and Sablayrolles, Alexandre and J{\'e}gou, Herv{\'e}},
  journal={arXiv preprint arXiv:2012.12877},
  year={2020}
}
@article{zhao2020point,
  title={Point transformer},
  author={Zhao, Hengshuang and Jiang, Li and Jia, Jiaya and Torr, Philip and Koltun, Vladlen},
  journal={arXiv preprint arXiv:2012.09164},
  year={2020}
}
@article{zheng2020rethinking,
  title={Rethinking Semantic Segmentation from a Sequence-to-Sequence Perspective with Transformers},
  author={Zheng, Sixiao and Lu, Jiachen and Zhao, Hengshuang and Zhu, Xiatian and Luo, Zekun and Wang, Yabiao and Fu, Yanwei and Feng, Jianfeng and Xiang, Tao and Torr, Philip HS and others},
  journal={arXiv preprint arXiv:2012.15840},
  year={2020}
}
@article{bertasius2021space,
  title={Is Space-Time Attention All You Need for Video Understanding?},
  author={Bertasius, Gedas and Wang, Heng and Torresani, Lorenzo},
  journal={arXiv preprint arXiv:2102.05095},
  year={2021}
}
@article{sharir2021image,
  title={An Image is Worth 16x16 Words, What is a Video Worth?},
  author={Sharir, Gilad and Noy, Asaf and Zelnik-Manor, Lihi},
  journal={arXiv preprint arXiv:2103.13915},
  year={2021}
}
@article{vivit,
  title={ViViT: A Video Vision Transformer},
  author={Arnab, Anurag and Dehghani, Mostafa and Heigold, Georg and Sun, Chen and Lu{\v{c}}i{\'c}, Mario and Schmid, Cordelia},
  journal={arXiv preprint arXiv:2103.15691},
  year={2021}
}
@article{xiang2017posecnn,
  title={Posecnn: A convolutional neural network for 6d object pose estimation in cluttered scenes},
  author={Xiang, Yu and Schmidt, Tanner and Narayanan, Venkatraman and Fox, Dieter},
  journal={arXiv preprint arXiv:1711.00199},
  year={2017}
}
@inproceedings{chen2024training,
  title={Training-free layout control with cross-attention guidance},
  author={Chen, Minghao and Laina, Iro and Vedaldi, Andrea},
  booktitle={WACV},
  year={2024}
}
@article{he2023mlanet,
  title={MLANet: Multi-Level Attention Network with Sub-instruction for Continuous Vision-and-Language Navigation},
  author={He, Zongtao and Wang, Liuyi and Li, Shu and Yan, Qingqing and Liu, Chengju and Chen, Qijun},
  journal={arXiv preprint arXiv:2303.01396},
  year={2023}
}
@article{kewenig2023evidence,
  title={Evidence of Human-Like Visual-Linguistic Integration in Multimodal Large Language Models During Predictive Language Processing},
  author={Kewenig, Viktor and Edwards, Christopher and DEstalenx, Quitterie Lacome and Rechardt, Akilles and Skipper, Jeremy I and Vigliocco, Gabriella},
  journal={arXiv preprint arXiv:2308.06035},
  year={2023}
}
@inproceedings{nasiriany2022augmenting,
  title={Augmenting reinforcement learning with behavior primitives for diverse manipulation tasks},
  author={Nasiriany, Soroush and Liu, Huihan and Zhu, Yuke},
  booktitle={ICRA},
  year={2022}
}
@inproceedings{yu2020meta,
  title={Meta-world: A benchmark and evaluation for multi-task and meta reinforcement learning},
  author={Yu, Tianhe and Quillen, Deirdre and He, Zhanpeng and Julian, Ryan and Hausman, Karol and Finn, Chelsea and Levine, Sergey},
  booktitle={CoRL},
  year={2020},
}
@inproceedings{pedersen2020grasping,
  title={Grasping unknown objects by coupling deep reinforcement learning, generative adversarial networks, and visual servoing},
  author={Pedersen, Ole-Magnus and Misimi, Ekrem and Chaumette, Fran{\c{c}}ois},
  booktitle={ICRA},
  year={2020},
}
@article{ren2015faster,
  title={Faster r-cnn: Towards real-time object detection with region proposal networks},
  author={Ren, Shaoqing and He, Kaiming and Girshick, Ross and Sun, Jian},
  journal={NeurIPS},
  year={2015}
}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%



% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor

\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}

\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.


\let\ab\allowbreak

